PromptAgent: Strategic Planning with Language Models Enables Expert-level Prompt Optimization

Highly effective, task-specific prompts are often heavily engineered by experts to integrate detailed instructions and domain insights based on a deep understanding of both instincts of large language models (LLMs) and the intricacies of the target task. However, automating the generation of such expert-level prompts remains elusive. Existing prompt optimization methods tend to overlook the depth of domain knowledge and struggle to efficiently explore the vast space of expert-level prompts. Addressing this, we present PromptAgent, an optimization method that autonomously crafts prompts equivalent in quality to those handcrafted by experts. At its core, PromptAgent views prompt optimization as a strategic planning problem and employs a principled planning algorithm, rooted in Monte Carlo tree search, to strategically navigate the expert-level prompt space. Inspired by human-like trial-and-error exploration, PromptAgent induces precise expert-level insights and in-depth instructions by reflecting on model errors and generating constructive error feedback. Such a novel framework allows the agent to iteratively examine intermediate prompts (states), refine them based on error feedbacks (actions), simulate future rewards, and search for high-reward paths leading to expert prompts. We apply PromptAgent to 12 tasks spanning three practical domains: BIG-Bench Hard (BBH), as well as domain-specific and general NLP tasks, showing it significantly outperforms strong Chain-of-Thought and recent prompt optimization baselines. Extensive analyses emphasize its capability to craft expert-level, detailed, and domain-insightful prompts with great efficiency and generalizability.

==> Tables/prompt_compare/highlight_caption.tex <==
\nolinebreak
including normal human prompt, APE-optimized prompt, and expert-level prompt optimized by PromptAgent. Both baselines mostly describe the task, while our expert prompt is composed of more complex structures and domain-specific insights, achieving superior performance. {Bold text} denotes \textbf{domain knowledge} usually handcrafted by domain specialists, but here automatically discovered by \ours. We highlight different aspects of expert prompt with colors, including \ctext[RGB]{233,252,232}{Task Description}, \ctext[RGB]{255,230,230}{Term Clarification}, \ctext[RGB]{230,246,255}{Solution Guidance}, \ctext[RGB]{255,230,200}{Exception Handling}, \ctext[RGB]{255,225,255}{Priority \& Emphasis}, \ctext[RGB]{230, 230, 255}{Formatting}. (Best view with colors)
